Log-based Anomaly Detection with Deep Learning: How Far Are We?

Software-intensive systems produce logs for troubleshooting purposes. Recently, many deep learning models have been proposed to automatically detect system anomalies based on log data. These models typically claim very high detection accuracy. For example, most models report an F-measure greater than 0.9 on the commonly-used HDFS dataset. To achieve a profound understanding of how far we are from solving the problem of log-based anomaly detection, in this paper, we conduct an in-depth analysis of five state-of-the-art deep learning-based models for detecting system anomalies on four public log datasets. Our experiments focus on several aspects of model evaluation, including training data selection, data grouping, class distribution, data noise, and early detection ability. Our results point out that all these aspects have significant impact on the evaluation, and that all the studied models do not always work well. The problem of log-based anomaly detection has not been solved yet. Based on our findings, we also suggest possible future work.

==> sections/experimental_setup.tex <==
\subsection{Datasets}
To evaluate the state-of-the-art in log-based anomaly detection, we select four public datasets\footnote{\url{https://github.com/logpai/loghub}}, namely HDFS, Blue Gene/L, Thunderbird, and Spirit. The details of each dataset are as follows:
\begin{itemize}
    \item \textit{HDFS:} HDFS dataset is produced from more than 200 Amazon EC2 nodes. In total, the HDFS dataset consists of 11,175,629 log messages. These log messages form different log windows according to their \textit{block\_id}, reflecting a program execution in the HDFS system, e.g., writing a file and then closing it. There are 575,061 blocks of logs in this dataset, among which about 2.93\% indicate system anomalies.
    \item \textit{BGL:} BGL dataset is a supercomputing system log dataset collected by Lawrence Livermore National Labs (LLNL) \cite{oliner2007supercomputers}. The BGL dataset contains 4,747,963 log messages. Each message in the BGL dataset was manually labelled as either normal or anomalous. There are 348,460 log messages that were labelled as anomalous, accounting for 7.34\% of logs.%\hy{how many percentages?}.
    \item \textit{Thunderbird:} Thunderbird is an open dataset of logs collected from a Thunderbird supercomputer at Sandia National Labs (SNL) \cite{oliner2007supercomputers}. The log contains normal and abnormal messages which are manually identified. Thunderbird is a large dataset of more than 200 million log messages. We leverage 10 million continuous log lines for computation-time purposes, which contains 4,934 anomalies according to the timestamps, accounting for 0.49\% of logs.%\hy{how many percentages?}.
    \item \textit{Spirit:} Similar to the Thunderbird log, the Spirit log is also an aggregation of system log data from the Spirit supercomputer system at Sandia National Labs \cite{oliner2007supercomputers}. There are more than 172 million log messages labeled as anomalous on the Spirit dataset. In this paper, we use a small set containing the first 5 million log lines of the original Spirit dataset, among which about 15.30\% indicate anomalies.%\hy{how many anomalies?}
\end{itemize}

\hy{need a table to summarize the data, including training and testing, and show the percentage of anomalies}
% \subsection{Experimental Models}

% In this study, we select the models to be evaluated according to the following criteria: (1) source code is publicly available, and (2) we can confirm the correctness of source code by checking the implementation provided by the authors and reproducing results presented in the original paper.

\subsection{Research Questions}
The goal of this study is to analyze the performance of the representative works on log-based anomaly detection (e.g., DeepLog or LogRobust). We design four research questions:

\textbf{1) RQ1: }\textit{How good are the existing approaches perform with different training data selection?} 

We want to evaluate whether or not  state-of-the-art tools are able to achieve good accuracy with different training data selection strategies. %different real-world datasets, including BGL, Thunderbird, and Spirit datasets. 
To this end, we conduct experiments with two different strategies for training data selection, including:
\begin{itemize}
    \item Random selection: For each dataset, we first sort logs by their timestamps, and then apply the fixed window grouping technique to generate log windows (i.e., instances)\hy{not clear 'log window', is it log sequences?also, make the term consistent with Figure 1}. Next, these instances are shuffled, and split into training/testing sets with the ratio of 80:20.
    \item Chronological selection: For each dataset, we utilize the first 80\% of raw logs (that appear in chronological order) for training and the remaining 20\% for testing. Next, we apply the fixed window grouping technique to generate log sequences. In this way, we can guarantee that only historical logs are used in the training phase and there is no future logs used in this phase.
\end{itemize}
In this RQ, we experiment on the BGL, Thunderbird, and Spirit datasets. As the HDFS dataset does not contain timestamp information, it is not used in this RQ. The value of window size for fixed window grouping is set to 1 hour.

\textbf{3) RQ2: }\textit{How do the existing models perform with different data grouping methods?}




\textbf{3) RQ3: }\textit{Can existing approaches work with different degrees of data noise?}

The noise of data is measured in terms of mismatched log ratio. To evaluate the impact of mismatched logs on the performance of DL-based methods, we randomly add a piece of anomalies (from 1\% to 20\%) into the training data for semi-supervised methods. For supervised methods, we randomly change the label of a specific portion (from 1\% to 20\%) to simulate the mismatched logs' scenarios. 

Moreover, to measure the impact of noises from log parsing errors, we experiment on four commonly used log parsers, including Drain \cite{he2017drain}, Spell \cite{du2016spell}, AEL \cite{jiang2008abstracting}, IPLoM \cite{makanju2009clustering}.

\textbf{4) RQ4: }\textit{How much early do the existing models detect anomalies in online detection?}
% \begin{tcolorbox}
% \textbf{Summary.} summary of the finding
% \end{tcolorbox}

\textbf{5) RQ5: }\textit{How effective are existing approaches under different settings?}

% \begin{tcolorbox}
% \textbf{Summary.} summary of the finding
% \end{tcolorbox}

\subsection{Evaluation Metrics}
To measure the effectiveness of \tool in anomaly detection, we use the Precision, Recall, Specificity, and F1-Score metrics, which are defined as follows:

\begin{itemize}
    \item \textit{Precision:} the percentage of correctly detected abnormal log sequences amongst all detected abnormal log sequences by the model. $Prec = \frac{TP}{TP + FP}$.
    \item \textit{Recall:} the percentage of log sequences that are correctly identified as anomalies over all real anomalies. $Rec = \frac{TP}{TP + FN}$.
    \item \textit{Specificity}: the percentage of log sequences that are correctly identified normal over all real normal sequences. $Spec=\frac{TN}{TN + FP}$ %\hy{this is proposed by us in this paper, so can describe it in corresponding RQ. The other three metrics are commonly used in existing work}
    \item \textit{F-Measure:} the harmonic mean of \textit{Precision} and \textit{Recall}.\\ $F1 = \frac{2 * Prec * Rec}{Prec + Rec}$
\end{itemize}
TP (True Positive) is the number of abnormal log sequences the are correctly detected by the model. FP (False Positive) is the number of normal log sequences that are wrongly identified as anomalies. FN (False Negative) is the number of abnormal log sequences that are not detected by the model.

\subsection{Experiment Setup}
